Beyond Prompts: Exploring the Design Space of Mixed-Initiative Co-Creativity Systems

Generative Artificial Intelligence systems have been developed for image, code, story, and game generation with the goal of facilitating human creativity. Recent work on neural generative systems has emphasized one particular means of interacting with AI systems: the user provides a specification, usually in the form of prompts, and the AI system generates the content. However, there are other configurations of human and AI coordination, such as co-creativity (CC) in which both human and AI systems can contribute to content creation, and mixed-initiative (MI) in which both human and AI systems can initiate content changes. In this paper, we define a hypothetical human-AI configuration design space consisting of different means for humans and AI systems to communicate creative intent to each other. We conduct a human participant study with 185 participants to understand how users want to interact with differently configured MI-CC systems. We find out that MI-CC systems with more extensive coverage of the design space are rated higher or on par on a variety of creative and goal-completion metrics, demonstrating that wider coverage of the design space can improve user experience and achievement when using the system; Preference varies greatly between expertise groups, suggesting the development of adaptive, personalized MI-CC systems; Participants identified new design space dimensions including scrutability -- the ability to poke and prod at models -- and explainability.

==> test.tex <==
\begin{abstract}
    \begin{quote}
Generative Artificial Intelligence that learns to create a wide array of contents can help game designers in their development process; 
However, as "state-of-the-art" generative AI remain advice oriented, much is to be studied towards an ideal collaborative experience, which mixed-initiative co-creative (MI-CC) system will promote.
To stimulate the research toward better MI-CC systems, building on the definition of Control Communications as information exchanges between users and the AI system towards the contents, 
We show the effects of including or excluding different types of Control Communications on user experience and content generated, 
by building an experimental system
and conduct a preliminary study with participants with different level of expertise.
We find out that MI-CC systems with a larger coverage of design space of Control Communications are rated higher or on par with ablations on a variety of creative and goal-completion metrics by 185 human participants, demonstrating that more coverage of the design space of Control Communications fore a MI-CC system has the potential to improve user experience and achievement from using the system;
Preference also varies greatly between demographic groups, suggesting at developing adaptive, personalized MI-CC systems.         
    \end{quote}
\end{abstract}



\section{Introduction}
With wider availability and affordability to generative AI systems in domains ranging from text\cite{brown_language_2020}, image\cite{ramesh_hierarchical_2022}, program code\footnote{https://github.com/features/copilot/}, to game contents\cite{khalifa_pcgrl_2020}, they have increasingly attracted attention from non-technical artists, writers, and content creators.
Although creators can now interact with such systems in a wide variety of ways, such as providing a prompt \cite{liu_pre-train_2021}, previous context \cite{brown_language_2020}, structured data \cite{lebret_neural_2016}, or even turn one kind of creative work into another \cite{radford_learning_2021}, 
the means of data input, along with the majority of interactions between these generation systems and the creators are not human-centered in that they impose paradigms of input on the human designer that is afforded by the underlying algorithms and models instead of the best suits the needs of the human designer;
as one would say "It's the model \textbf{teaching} 
\textit{you}, instead of you teaching the model".

To prevent greater cognitive load, frustration, and ultimately reduced use of a system 
\cite{sweller_cognitive_2011},
efforts including studies in AI Literacy \todo{cite}, embedding generators in familiar settings such as chat bots\todo{cite chatgpt}, and what we focus on in this work: to develop Mixed-Initiative Co-Creativity (MI-CC) systems.

MI-CC systems \cite{liapis_can_2016} systems (further introduced in Section \ref{subsection:related-micc}) are promising ways to improve the 

\todo{mixed-initiative co-creativity is a thing people are chasing, and is a promising way to solve this problem}

\todo{however, different kinds of information flow (we call it comm) is under studied}

\todo{Our contribution is to further formalize comms and highlight the importance of studying this by showing in many cases more comm is better}
In this paper, we 

\section{Background and Related Work}
\label{subsection:related-micc}
Mixed-initiative Co-creativity (MI-CC) systems are designed toward two goals: being \textit{mixed-initiative} and \textit{co-creative}.

A mixed-initiative system is one where ``a human initiative and a computational initiative" cooperate towards a shared goal~\cite{novick_what_1997}.
In this work, we focus on the game design domain~\cite{yannakakis_mixed-initiative_2014};
However, just as ~\cite{lai_mixed-initiative_2022} pointed out it can be easily applied to other creative domains.
Just like in ~\cite{lai_mixed-initiative_2022} we also take fire-and-forget systems out of this domain and focus on systems that allow iterative improvement on the creative artifact.

We refer to a {\em co-creative} \cite{rezwana_cofi_2021,rezwana_designing_2022,guzdial_interaction_2019,grabe_towards_2022,kreminski_reflective_2021} agent as one that ``possesses the ability to alter the creative work equal to a human counterpart".
Note that when it comes to capability, ability does not imply \textit{human-parity}.
Furthermore, as the human user and the AI system may tackle different parts of the creative work, it also does not entail \textit{responsibility}.

A mixed-initiative system does not necessarily need to be co-creative as the final product of the process does not have to be a creative artifact \cite{sekulic_evaluating_2022};
However, it is an appealing goal for mixed-initiative systems to be co-creative ~\cite{lai_mixed-initiative_2022}.

To study the information that flows between the user and the MI-CC agent (See Section \ref{subsection:communication}), we expanded on the definition of Communications from \cite{lin_creative_2022},
which is itself based off previous effort in categorizing or differentiating between different types of interactions between these parties;
This includes \cite{rezwana_cofi_2021,rezwana_designing_2022}, a framework that models interactions in co-creative systems that ``focus on flow of information between collaborators'', inspiring the definition of Communications;
\cite{guzdial_interaction_2019}, which inspires the human-vs-agent-initiated dimension by pointing out that human designers and AI ``can initiate the same action sets to modify the creative work, albeit with different executions'';
and \cite{kreminski_reflective_2021}, which inspires the elaboration vs. reflection dimension by presenting a survey on communications ``where the agent thinks about what happened in the process and takes actions based on it''.

Recent works on co-creative systems with a large array of interactive options includes CoAuthor \cite{lee_coauthor_2022}, where in a text continuation setting fine-grained keyboard-based actions are recorded as a dataset; 
and CoPoet \cite{chakrabarty_help_2022}, which in a poetry domain, options are implemented as prompts constructed to represent requests with different level of specificity and range of application.
These work has shown the potential of co-creativity systems (note that none of them is mixed-initiative by design) with a wide range of capabilities, further encouraging us on a comparative study over the design space of these capabilities, which is the focus of this work.

\section{\textit{Communications} in mixed-initiative co-creative systems}
\subsection{What \textit{exactly} is Communications?}
\label{subsection:communication}
MI-CC systems come in a variety of sizes and shapes.
\cite{lin_creative_2022} formalized abstraction of MI-CC systems;
Their abstraction can well represent these differences, ranging from creative domains the system works on, the style of representation of the information (visual, textual, etc.), how information flows between the system and its users, to how this is controlled chronologically.
In this work, we focus on one dimension of differences MI-CC systems have: the flow of information, or as defined in \cite{lin_creative_2022}, \textit{Communications}.

To concisely study Communications, we decouple them from the representations of related information, which sometimes are also referred to as communications, so as to focus on the information flow itself.
Although one can argue that a MI-CC system can have "textual Communications" along with visual (and any other types of them) ones, and this changes the behavior and perception of the systems \cite{margarido_lets_2022} and we acknowledge that this is a promising field to study, we deem this as out of the scope of this work.

Expanding on the definition of Communications in \cite{lin_creative_2022}, we identify that information that flows between the user and the AI does not have to relate to improving what is being created, just like collaborations between people.
For example, one can say "hello" to their counterparts, acknowledge good ideas, explain their reason for making certain decisions, or chat about random things;
We term them \textbf{Social} Communications.
Although these communications do not necessarily reduce the productivity of collaboration,
and instead may improve the relationship between users and the AI agent, allow users to better understand the AI system, and improve trustworthiness \cite{margarido_lets_2022},
in this paper, we focus on Communications that are not Social; 
We coin them \textbf{Control} Communications.

\textit{Definition - } Control Communications: Information exchange in a mixed-initiative co-creativity session that relates to potential changes in the creative artifact.

For the rest of this work, we abbreviate Control Communications to simply communications and concentrate on who is initializing them and what their target is, both from a content and chronological perspective.

\subsection{Why study the design space of Communications in a MI-CC context?}
\label{subsection:dimensions}
On one hand, recent generation systems, such as ChatGPT and Copilot \todo{cite cite}, demonstrate state-of-the-art capability when requested.
They can often retrieve information from the context they are working in, and provide useful suggestions based on both what is retrieved and their internal knowledge.
On the other hand, representations of collaborative information are relatively well studied, and many systems with different user interfaces enabling delivery in a wide variety of modals (textual, audio, visual, graphical, structured) \todo{cite cite} exists.
However, the choice of information actually provided and requested is under explored beyond fire-and-forget systems which are trained on text corpus and/or task-based human feedback \todo{cite davinci 002 003 and RLHF}.
We argue that this is because these cutting-edge "collaborative" systems are designed more towards being an "assistant"; although they are successful towards that goal, it does not align well with a better MI-CC experience.

With this recent trend in hindsight, \cite{kreminski_reflective_2021} pointed out that one of the additional roles of an MI-CC agent above question-answering is self-reflection; 
Furthermore, \cite{lin_creative_2022} proposed three continuous, non-exhaustive dimensions to classify communications into:
\begin{itemize}
    \item \textbf{Human-initiated vs. Agent-initiated}, which "considers which of the two parties is initiating communication";
    \item \textbf{Elaboration vs. Reflection}, which deals with "whether the communication relates to previously generated contents (reflection) or to newly planned actions (elaboration)";
    \item \textbf{Global vs. Local}, which is based on "the scope of the creative work" of the communication.
\end{itemize}
Studying MI-CC systems with Communications from different parts of the design space will help researchers to better understand how an AI system will collaborate with a human designer and facilitate cutting-edge generation systems to better align with tasks unique to MI-CC systems. 



\section{Experiment design}
To study the design space of Communications, we designed and conducted a study comparing systems with different coverage of the design space formulated in Section \ref{subsection:communication}.
We establish the following hypothesis:
\begin{itemize}
    \item \textbf{H1}: Users will prefer an MI-CC system that provides Control Communications (See Section \ref{subsection:communication} that covers a larger subspace in the design space (See Section \ref{subsection:dimensions};
    \item \textbf{H2}: Users who have different levels of expertise in creating using a computer in general and domain-specifically, and at various level of AI Literacy, will also have varied preference over MI-CC systems.
\end{itemize}
This study consists of a participant answering questions in a survey and using both the "Full" system and one ablation.

In this section, we will describe the design of the study based on this hypothesis; In section \ref{section:exp-sys} we will illustrate our experimental systems and ablations used for the study.

\subsection{Survey Design}
\label{subsection:survey-design}
We first ask participants to self evaluate their \Zhiyu{If we get space eveutually I will explain what these levels are} 
\begin{itemize}
    \item Level of confidence with using a computer to author contents (rated from A1 to A4);
    \item Level of confidence with using a computer to create games (rated from B1 to B4);
    \item Familiarity with AI (rated from C1 to C3).
\end{itemize}

We then show instructions to familiarize them with the interface of the experiment system;
Once they've finished reading the instruction, they are randomly \footnote{balanced sampling; participants get assigned to each group with the same chance.} assigned to an ablation group and prompted to use both the "Full" system and the ablation system (one from 6 available, described in Section \ref{subsection:ablations});
We counter-balanced the presentation of the systems so that participants randomly start with using either "Full" or the ablation system.

To facilitate the creative experiment, we assigned the same goal that \cite{lin_creative_2022} used, which is to generate a story that starts with "Business" and ends in "Sports" while mentioning "soccer".
The participants are given 12 turns for each system, counted in successful interactions. \footnote{At any time the user can opt to not commit the changes and cancel out of a Communication, not taking a turn.}

Once they finished using both systems, as the exit survey, we asked 7 questions about their satisfaction with the process and the generated story.
They are randomly ordered for each participant.

The first 6 questions are adapted from the Creative Support Index (CSI) by \cite{cherry_quantifying_2014}, which is an index that is designed to measure "how well a tool is supporting creativity".
We ask, between the "Full" system and the ablation participant got assigned, "Which system is more associated with each of the statements?":
\begin{itemize}
    \item Q1: \textbf{(Expressiveness)} This system made it easiest for me to express and share my goals, given to me in instructions, with the AI system.
    \item Q2: \textbf{(Enjoyment)} I enjoyed interacting with this system most.
    \item Q3: \textbf{(Exploration)} This system was most helpful for exploring different ideas and possibilities.
    \item Q4: \textbf{(Immersion)} This system made me feel the most absorbed in the task to the point that I forgot I was working with the system.
    \item Q5: \textbf{(Collaboration)} This system best allowed me to achieve the goal assigned to me.
    \item Q6: \textbf{(Results worth effort)} This system provides the overall best quality stories by the time I was done.
\end{itemize}

Additionally, we also asked Q7: (Which system tends to) "get the best response for the same type of requests".
We anticipate no preference between both systems on Q7, as the implementations of how the systems handles these requests (i.e. what is described in Section \ref{subsection:comm_instantiation}), provide that an ablation system has that capacity, are exactly the same.

As an attention mechanism, We also asked what the perceived similarity and differences between these two systems are before the participant finishes the study.

\section{Experimental System Overview}
\label{section:exp-sys}
To study the assumptions we have, we built an experimental system using the Creative Wand framework \cite{lin_creative_2022}.
This framework outlines a MI-CC system to have 4 major components:
\begin{itemize}
    \item Creative Context, which interfaces to the generative and any other algorithms related to the specific domain;
    \item Experience Manager, which is responsible for maintaining the state of the system;
    \item Communications, which instantiates \textit{Communications} described in \ref{subsection:comm_instantiation};
    \item Frontend, which defines the representation of information between the system and the human designer.
\end{itemize}

Table \ref{table:instantiation} provides an overview of the story creation system we used for our experimental system.

\begin{table*}[htbp]
\centering
\begin{tabular}{c|p{0.8\linewidth}} 
\toprule
{\bf Module} & {\bf Description} \\ 
\hline
{\bf CreativeContext}    & Language Models that generates 10-sentence stories and provides other services. \\ 
\hline
{\bf ExperienceManager}  & A turn and rule-based agent that keeps system states and present communications based on context.~              \\ 
\hline
{\bf Frontend} & A React.js web application with a canvas and chatbox interface.                                                                           \\
\hline
{\bf Communications} & Control and Social communications (See TODO for details)                                                                            \\
\bottomrule
\end{tabular}
\caption{Summary of Creative Wand instantiations used in the experiment.}
\label{table:instantiation}
\end{table*}





\bibliographystyle{iccc}
\bibliography{references}
